Analyzing General-Purpose Deep-Learning Detection and Segmentation Models with Images from a Lidar as a Camera Sensor

Over the last decade, robotic perception algorithms have significantly benefited from the rapid advances in deep learning (DL). Indeed, a significant amount of the autonomy stack of different commercial and research platforms relies on DL for situational awareness, especially vision sensors. This work explores the potential of general-purpose DL perception algorithms, specifically detection and segmentation neural networks, for processing image-like outputs of advanced lidar sensors. Rather than processing the three-dimensional point cloud data, this is, to the best of our knowledge, the first work to focus on low-resolution images with 360\textdegree field of view obtained with lidar sensors by encoding either depth, reflectivity, or near-infrared light in the image pixels. We show that with adequate preprocessing, general-purpose DL models can process these images, opening the door to their usage in environmental conditions where vision sensors present inherent limitations. We provide both a qualitative and quantitative analysis of the performance of a variety of neural network architectures. We believe that using DL models built for visual cameras offers significant advantages due to the much wider availability and maturity compared to point cloud-based perception.

==> sec/05_Discussion.tex <==


\section{Discussion}

The results from our experiments demonstrate the potential of lidars as camera sensors with out-of-the-box, state-of-the-art DL-based perception models. Indeed, this type of data processing pipeline comes at no extra costs for autonomous systems where lidars are already present. 

The positive performance of both object detectors and semantic instance segmentation networks opens the door to broader use of these sensors for perception beyond the analysis of the three-dimensional point clouds. Our work extends the results from previous experiments in~\cite{tsiourva2020lidar} that already show the potential of the lidars as cameras, especially in adverse weather conditions and environments where passive vision sensors present inherent limitations.

Among the applications of lidars as cameras in autonomous robotic solutions is their potential for odometry estimations and aiding both lidar and visual odometry with an intrinsically multi-modal data source. This has been loosely explored in~\cite{angus2018lidar}, but further research is needed to quantify the performance of such an approach.

One aspect that also requires further study is utilising the different images generated by the lidar sensors. Through this work, we decided to focus on one of the three types of images provided by the lidars, namely the signal image. In addition to it, the sensors also provide depth, near-infrared and reflectivity images. These, however, do not perform as well with out-of-the-box DL models without further pre-processing, as we illustrate with a sample in Fig.~\ref{fig:yolox_images_compare} and Fig.~\ref{fig:yolox_0}. One option to be further explored in the future is the combination of these images as multiple channels of a single image.

\begin{figure}
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=.95\textwidth,height=0.2\textwidth]{fig/comparison/pic1.jpeg}
        \caption{YOLOx detection results on on a sample image from the near-infrared channel.}
        \label{fig:yolox_nearir}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=.95\textwidth,height=0.2\textwidth]{fig/comparison/pic2.jpeg}
        \caption{YOLOx detection results on a sample image from the reflectivity channel.}
        \label{fig:yolox_reflec}
    \end{subfigure}
    %  \begin{subfigure}{\textwidth}
    %     \includegraphics[width=.95\textwidth]{}
    %     \caption{Caption}
    %     \label{fig:my_label}
    % \end{subfigure}
    \caption{YOLOx Detection Based on Images from Other Channels of Ouster Lidar}
    \label{fig:yolox_images_compare}
\end{figure}
